On Retrospective k-space Subsampling schemes For Deep MRI Reconstruction

Acquiring fully-sampled MRI $k$-space data is time-consuming, and collecting accelerated data can reduce the acquisition time. Employing 2D Cartesian-rectilinear subsampling schemes is a conventional approach for accelerated acquisitions; however, this often results in imprecise reconstructions, even with the use of Deep Learning (DL), especially at high acceleration factors. Non-rectilinear or non-Cartesian trajectories can be implemented in MRI scanners as alternative subsampling options. This work investigates the impact of the $k$-space subsampling scheme on the quality of reconstructed accelerated MRI measurements produced by trained DL models. The Recurrent Variational Network (RecurrentVarNet) was used as the DL-based MRI-reconstruction architecture. Cartesian, fully-sampled multi-coil $k$-space measurements from three datasets were retrospectively subsampled with different accelerations using eight distinct subsampling schemes: four Cartesian-rectilinear, two Cartesian non-rectilinear, and two non-Cartesian. Experiments were conducted in two frameworks: scheme-specific, where a distinct model was trained and evaluated for each dataset-subsampling scheme pair, and multi-scheme, where for each dataset a single model was trained on data randomly subsampled by any of the eight schemes and evaluated on data subsampled by all schemes. In both frameworks, RecurrentVarNets trained and evaluated on non-rectilinearly subsampled data demonstrated superior performance, particularly for high accelerations. In the multi-scheme setting, reconstruction performance on rectilinearly subsampled data improved when compared to the scheme-specific experiments. Our findings demonstrate the potential for using DL-based methods, trained on non-rectilinearly subsampled measurements, to optimize scan time and image quality.

==> supporting.tex <==
\section*{Supporting information}
The following supporting information is available as part of the online article:

\vskip\baselineskip\noindent
\textbf{Figure S1.}
\xlabel{fig:S1}
{Representative reconstruction of a sample from the Calgary Campinas test set obtained from the scheme-specific experiments.}

\noindent
\textbf{Figure S2.}
\xlabel{fig:S2}
{Scheme-specific setup vs multi-scheme setup quantitative results comparison. Violin-plots illustrate the evaluation metric differences between the reconstructed output of the model trained on all subsampling schemes (multi-scheme) and the reconstructed output of the model trained on a single scheme (scheme-specific).}

\noindent
\textbf{Figure S3.}
\xlabel{fig:S3}
{Scheme-specific vs multi-scheme setups visual comparison. Representative reconstructions of a sample from the Calgary-Campinas dataset subsampled with the four rectilinear schemes obtained from the scheme-specific and multi-scheme experiments for three acceleration factors.}

\noindent
\textbf{Figure S4.}
\xlabel{fig:S4}
{Model dependence experiments quantitative results on the Calgary-Campinas dataset using RIMs instead of RecurrentVarNets.}


\noindent
\textbf{Table S1.}
\xlabel{tab:S1}
{Acquisition parameters and experiment splits per dataset used in our experiments.}

\noindent
\textbf{Table S2.}
\xlabel{tab:S2}
{Scheme-specific experiments average results on the test sets. 
% Bold numbers indicate the best across subsampling schemes.
}


\noindent
\textbf{Table S3.}
\xlabel{tab:S3}
{Multi-scheme experiments average results on the test sets.
% Bold numbers indicate the best across subsampling schemes.
}

\noindent
\textbf{Table S4.}
\xlabel{tab:S4}
{Model dependence experiments average quantitative results on the Calgary-Campinas dataset using RIMs instead of RecurrentVarNets.
% Bold numbers indicate the best across subsampling schemes.
}
